Learning Rhythmic Trajectories with Geometric Constraints for Laser-Based Skincare Procedures

The increasing deployment of robots has significantly enhanced the automation levels across a wide and diverse range of industries. This paper investigates the automation challenges of laser-based dermatology procedures in the beauty industry; This group of related manipulation tasks involves delivering energy from a cosmetic laser onto the skin with repetitive patterns. To automate this procedure, we propose to use a robotic manipulator and endow it with the dexterity of a skilled dermatology practitioner through a learning-from-demonstration framework. To ensure that the cosmetic laser can properly deliver the energy onto the skin surface of an individual, we develop a novel structured prediction-based imitation learning algorithm with the merit of handling geometric constraints. Notably, our proposed algorithm effectively tackles the imitation challenges associated with quasi-periodic motions, a common feature of many laser-based cosmetic tasks. The conducted real-world experiments illustrate the performance of our robotic beautician in mimicking realistic dermatological procedures; Our new method is shown to not only replicate the rhythmic movements from the provided demonstrations but also to adapt the acquired skills to previously unseen scenarios and subjects.

==> Docs/Biography.tex <==
\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/Anqing}}]
	{Anqing Duan} received the bachelor's degree in mechanical engineering from Harbin Institute of Technology, China, in 2015, the master's degree in mechatronics from KTH, Sweden, in 2017, and the Ph.D. degree in robotics from the Istituto Italiano di Tecnologia and the Università degli Studi di Genova, Italy, in 2021. He was a visiting researcher with the Learning Algorithms and Systems Laboratory at Swiss Federal Institute of Technology Lausanne, Switzerland. 
Since 2021, he has been a Research Associate with the Robotics and Machine Intelligence Laboratory at The Hong Kong Polytechnic University, Hong Kong. 
His current research interest lies in the intersection of machine learning and robotics.
\end{IEEEbiography}

\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/lcwl.jpg}}]
	{Wanli Liuchen} received the B.Sc. degree in Mechanical Design Manufacture and Automation from China University of Petroleum - Beijing, China, in 2022. He is currently working toward the M.Sc. degree in Mechanical Engineering at The Hong Kong Polytechnic University, Hong Kong. His research interests include robot navigation and machine learning.
\end{IEEEbiography}

\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/Jinsong_resize.jpg}}]
	{Jinsong Wu} received the MRes degree in Medical Robotics and Image-Guided Intervention from Imperial College London, UK, in 2022. Since 2023, he has been pursuing a Ph.D. degree in mechanical engineering at The Hong Kong Polytechnic University, Hong Kong. His current research interests include medical robotics and control theory.
\end{IEEEbiography}

\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/RCamoriano_resize.jpg}}]
	{Raffaello Camoriano} (Member, IEEE) received the B.Sc. (cum laude) and M.Sc. degrees in computer and robotics engineering and the Ph.D. degree from the University of Genoa, Italy, in 2011, 2013, and 2017, respectively. He has been a Research Fellow and a Postdoctoral Researcher at the Istituto Italiano di Tecnologia, Genoa, Italy, from 2014 to 2022. He is currently an Assistant Professor with the Department of Control and Computer Engineering at Politecnico di Torino, Turin, Italy, and an Affiliated Researcher at Istituto Italiano di Tecnologia.

    He is author of 20 international peer-reviewed articles in the fields of efficient learning from structured data, continual learning, reinforcement learning, and robotics. Prof. Camoriano received the IEEE Computational Intelligence Society Italy Section Chapter’s 2017 Best Ph.D. Thesis Award and is a Member of the European Laboratory for Learning and Intelligent Systems. He serves as an Associate Editor of the \textsc{IEEE Robotics and Automation Letters} and of the \textsc{IEEE/RSJ International Conference on Intelligent Robots and Systems}.
\end{IEEEbiography}

\begin{IEEEbiography} [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/Lorenzo}}]
	{Lorenzo Rosasco} received the Ph.D. degree in computer science from the University of Genova, Genoa, Italy, in 2006.
He is currently a Full Professor with the University
of Genova, Genoa, Italy. He is also affiliated with the
Massachusetts Institute of Technology (MIT), Cambridge, MA, USA, where he is currently a Visiting
Professor, and with the Istituto Italiano di Tecnologia
(IIT), Genoa, where he is an External Collaborator.
He is leading the efforts to establish the Laboratory
for Computational and Statistical Learning, from a
collaborative agreement between IIT and MIT. Between 2006 and 2009, he was
a Postdoctoral Fellow with Center for Biological and Computational Learning,
MIT, working with T. Poggio. His research interests include theory and algorithms for machine learning. He has developed and analyzed methods to learn from small as well as large samples of high-dimensional data, using analytical and probabilistic tools, within a multidisciplinary approach drawing concepts and techniques primarily from computer science but also from statistics, engineering, and applied mathematics.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{AuthorPhoto/david.jpg}}] {David Navarro-Alarcon} (Senior Member, IEEE) received the master's degree in robotics from the Centre for Research and Advanced Studies, National Polytechnic Institute of Mexico, in 2009, and the Ph.D. degree in mechanical and automation engineering from The Chinese University of Hong Kong (CUHK), Hong Kong, in 2014.
From 2015 to 2017, he was a Research Assistant Professor at the CUHK T Stone Robotics Institute, Hong Kong.
Since 2017, he has been with The Hong Kong Polytechnic University (PolyU), Hong Kong, where he is currently an Associate Professor with the Department of Mechanical Engineering, and the Principal Investigator of the Robotics and Machine Intelligence Laboratory.
His research interests include perceptual robotics and control theory. 
He currently serves as an Associate Editor of the \textsc{IEEE Transactions on Robotics} and Associate Editor of the \textsc{IEEE Robotics and Automation Magazine}.
\end{IEEEbiography}

==> Docs/FaceModel.tex <==
% We first construct a face surface manifold from point cloud data (Section \ref{face_model}).
% \subsection{Modeling of Face Surface}
% \label{face_model}
In order to identify the surface manifold that hosts the demonstrated trajectories of the laser gun, we first consider constructing a parametric surface model that can describe a human's face.
The purpose of parameterizing the human face surface is threefold: \romannumeral 1) it provides a trackable constraint on trajectory evolution of the laser gun; \romannumeral 2) it simplifies trajectory adaptation for treating a new patient's face by taking into account the surface parameters only, and \romannumeral 3) it enables smooth laser gun orientation control as normal vectors directly obtained from point cloud data could be jittering.  
To retrieve the parameters of a human face surface, we first need to collect the corresponding point cloud points of the human face.
By using a commercial depth camera, the captured cloud points dataset is formed as $\mathbb{D}_p: \{\boldsymbol{\xi}_n^p = (x^p_n, y_n^p, z_n^p) \}_{n=1}^{N}$ where the position of each point is expressed with respect to the coordinate $\mathcal{O}-xyz$. 
Before proceeding to parameterize the face surface, we first re-orient the collected face points such that in the Cartesian space we can parameterize the face surface as $(x, y, z(x, y))$.
Specifically, we would like the projected area of the face surface onto the $x-y$ plane to be maximized. 
One feasible approach is to calculate the principle components of the data points and make the first two components aligned with $x-$ and $y-$axis, respectively \cite{jolliffe2016principal}.
The third one should be aligned with either positive or negative direction of the $z-$axis such that the bundle of norms of the face surface can point towards the positive direction of the $z-$axis. 
To this end, we first compute the data covariance matrix $\boldsymbol{\Sigma}^p$ of the points in $\mathbb{D}_p$:
\begin{equation*}
\boldsymbol{\Sigma}^p = \frac{1}{N}\sum_{n=1}^{N}(\boldsymbol{\xi}_n^p-\overline{\boldsymbol{\xi}^p})(\boldsymbol{\xi}_n^p-\overline{\boldsymbol{\xi}^p})^\top \; \text{with} \;\; \overline{\boldsymbol{\xi}^p} = \frac{1}{N}\sum_{n=1}^{N}\boldsymbol{\xi}_n^p
\end{equation*}
Notably, the principle components of $\mathbb{D}_p$ are the eigenvectors of the data covariance matrix $\boldsymbol{\Sigma}^p$ in decreasing order, i.e. $\mathbf{v}_i=\mathrm{evec}_i(\boldsymbol{\Sigma}^p)$.
Consequently, the rotation matrix for re-orientation of the face surface with respect to the coordinate $\mathcal{O}$ can be constructed as
\begin{equation*}
~^\mathcal{O}\mathbf{R}_p =
    \begin{cases}
      [\mathbf{e}_1, \mathbf{e}_2, \mathbf{e}_3] & \mathbf{e}_3 \; \textrm{outwards,}\\
      [\mathbf{e}_2, \mathbf{e}_1, -\mathbf{e}_3] & \mathbf{e}_3 \; \textrm{inwards,}
    \end{cases} \quad
\text{with} \quad \mathbf{e}_i = \frac{\mathbf{v}_i}{\|\mathbf{v}_i\| }      
\end{equation*}
Finally, the coordinate of the  data points for the re-oriented face surface are calculated according to the homogeneous representation \cite{murray2017mathematical}:
\begin{equation*}
    \begin{bmatrix}
           \boldsymbol{\xi}_n^f \\
           1
    \end{bmatrix}=
    \begin{bmatrix}
           ~^\mathcal{O}\mathbf{R}_p^{-1} & -~^\mathcal{O}\mathbf{R}_p^{-1}\overline{\boldsymbol{\xi}^p} \\
           0 & 1
    \end{bmatrix}
    \begin{bmatrix}
           \boldsymbol{\xi}_n^p \\
           1
    \end{bmatrix}.
\end{equation*}
It should be noted that when performing cosmetic treatment for a patient, the end-effector of the robot should not touch the patient's skin.
In other words, a constant distance $d$ between the laser gun tip and the face surface is required.
Therefore, in order to construct the surface manifold on which the robot end-effector trajectory is constrained to evolve, we "inflate" the face surface by
$$\boldsymbol{\xi}_i = \boldsymbol{\xi}_i^f + d\mathbf{n}^f_i $$
where $\mathbf{n}^f_i$ is the normal vector for the $i$-th point $\boldsymbol{\xi}^f_i$.
As a result, the dataset from which we construct the surface manifold is collected as $\mathbb{D}_s: \{\boldsymbol{\xi}_n = (x_n, y_n, z_n)\}_{n=1}^N$.
Regarding selection of surface parameterization technique, it is desired that a large volume of points needed by data-driven approach is limited to a few "critical points" for surface representation.
Hence, free-form parametric methods are employed for surface parameterization which has gained popularity in computer graphics, computer-aided design, and finite element modeling.
In this paper, we consider to fit $\mathbb{D}_s$ to a Bézier surface though other free-form parametric approaches such as B-spline and non-uniform rational basis spline (NURBS) are very similar in principle and thus applicable as well \cite{farin2002handbook}.
The Bézier surface is determined as per $(M_x+1)\times(M_y+1)$ control points $\mathbb{C}: \{ \{\boldsymbol{\zeta}_{ix, iy} = (x_{ix}, y_{iy}, z_{ix, iy})\}_{ix=0}^{M_x} \}_{iy=0}^{M_y}$:
\begin{equation*}
	z(x, y) = \sum_{ix=0}^{Mx}\sum_{iy=0}^{My} B_{ix}^{Mx}(x_{ix}) B_{iy}^{My}(y_{iy})z_{ix, iy},
\end{equation*}
where the basis Bernstein polynomials are defined as 
\begin{equation*}
	B_i^M(x) =	\frac{M!}{i!(M-i)!}x^i(1-x)^{M-i}.
\end{equation*}

\cite{galvez2007bezier}

fitting to point cloud data genetic algorithms, functional networks and least-squares approximation 

least squares found out by appendix

